To Compute or not to Compute? Adaptive Smart Sensing in Resource-Constrained Edge Computing

We consider a network of smart sensors for an edge computing application that sample a time-varying signal and send updates to a base station for remote global monitoring. Sensors are equipped with sensing and compute, and can either send raw data or process them on-board before transmission. Limited hardware resources at the edge generate a fundamental latency-accuracy trade-off: raw measurements are inaccurate but timely, whereas accurate processed updates are available after processing delay. Hence, one needs to decide when sensors should transmit raw measurements or rely on local processing to maximize network monitoring performance. To tackle this sensing design problem, we model an estimation-theoretic optimization framework that embeds both computation and communication latency, and propose a Reinforcement Learning-based approach that dynamically allocates computational resources at each sensor. Effectiveness of our proposed approach is validated through numerical experiments motivated by smart sensing for the Internet of Drones and self-driving vehicles. In particular, we show that, under constrained computation at the base station, monitoring performance can be further improved by an online sensor selection.

==> Sections/RL-general.tex <==
%!TEX_root = ../processing_networks_estimation_RL.tex

\subsection{General Scenario}\label{sec:RL-general-scenario}

The Reinforcement Learning framework~\cite{Sutton1998} consists of an agent interacting
with an environment without having any prior knowledge of how the latter works and how its actions may impact on it.
By collecting results of the interactions, which are expressed through a reward signal,
the agent will learn to maximize this user-defined quantity, under the action of the unknown environment.
%In particular, in the problem under analysis, the base station will have the role of the agent, which tries different policies for the sensors in order to obtain the highest possible reward, defined as the negative average of the trace of the error covariance. \\
This can be formalized with the help of the Markov Decision Process framework,
in which the tuple $\left< \mathcal{S}, \mathcal{A}, \mathcal{P}, r, \gamma \right>$ characterize all needed elements,
\ie the state space $\mathcal{S}$;
the set of all possible actions $\mathcal{A}$;
the transition probabilities $\mathcal{P}$ regulating the underlying system, which may also be deterministic;
the reward function $r$, which is assumed to be a function of the state and the action;
and the discount factor $\gamma$, weighting future rewards.
The agent selects actions to be performed on the environment through a \textit{control policy},
which is here assumed to be a deterministic function $ \pi $ mapping states to actions, $\pi: \mathcal{S} \rightarrow \mathcal{A}$.
The goal of the learning procedure would be to identify an optimal policy $\pi^*(\cdot)$, 
\ie a map allowing to achieve the highest possible return $G$ over the long run,
according to the unknown transitions imposed by the environment.
The return is defined as the expectation of the sum of rewards in an episode of $K$ steps, 
\ie $G = \mathbb{E}\left[ \sum_{k=1}^K r_k \right]$. 
The general problem can be written as
\begin{maxi!}
	{\substack{\policy\in\Pi}}
	{\mathbb{E}_\pi\ls\sum_{k=0}^{K-1}\gamma^k r\lr s_k, a_k\rr\rs\protect\label{eq:RL-problem-objective}}
	{\label{eq:RL-problem}}
	{}
	\addConstraint{s_{k+1}^{\policy}}{= g\lr s_k, a_k \rr = g\lr s_k, \pi\lr s_k\rr\rr \doteq g_\pi\lr s_k\rr, \protect\label{eq:RL-problem-kalman}}
\end{maxi!}
where the state-transition function $g: \mathcal{S}\times\mathcal{A} \rightarrow \mathcal{S}$ 
representing environment dynamics that embeds the transition probabilities $\mathcal{P}$.
One of the simplest and most popular approaches to solve maximization~\eqref{eq:RL-problem} is the Q-learning algorithm \cite{Watkins1992}.

Q-learning is a \textit{model-free} algorithm which finds an optimal policy to maximize the expected value of the return, 
without learning an explicit model of the environment. 
This is done by focusing solely on the \textit{values} of actions at different states, which correspond to the return. 

In the tabular setting this method actually builds a lookup table with the action-value for each state-action pair,
and updates it with an \textit{optimistic} variant of the temporal-difference error~\cite{10.1023/A:1022633531479} at every step, 
weighted by a learning rate $\alpha$.

The action-value function is defined as
\begin{equation}
	Q^\pi(s, a) = \mathbb{E}_\pi\ls\sum_{k=0}^{K-1}\gamma^k r(s_k, a_k) \Bigg\vert s_k = s, a_k=a\rs,
\end{equation}
and it expresses the expected return obtained by performing action $a$ at state $ s $ and then following policy $\pi$ afterwards. \\
The Q-learning algorithm iteratively updates an estimate of the action-value function $\hat{Q}$, replacing the current estimate with the one given by the best performing action and bootstrapping for the future predictions.
By defining the optimistic variant of the temporal-difference error as
\begin{equation}
	\zeta^\pi_k \lr s, a\rr = r\lr s, a\rr + \gamma\max_{a'}\ls \hat{Q}_k \lr s',a'\rr\rs - \hat{Q}_k \lr s,a \rr,
\end{equation}
the update for the Q-learning algorithm is given by
\begin{equation}
	\hat{Q}_{k+1}\lr s,a\rr = 
	\begin{cases}
		\hat{Q}_k\lr s,a\rr + \alpha \, \zeta^\pi_k \lr s, a\rr \hfill \text{if } k<K-1, \\
		\lr1-\alpha\rr \hat{Q}_k\lr s,a\rr + \alpha \, r\lr s_k, a_k\rr \hfill \text{otherwise}.
	\end{cases}
\end{equation}
The Q-function is updated at each step $k = 1, 2, \dots$ of one episode. 
The policy deployed in the environment to run the episodes and collect rewards (\emph{behavioral policy})
is usually chosen as the $\epsilon$-greedy policy according to the current lookup table, 
emphasizing the explorative behavior of the algorithm.

In a finite MDP, 
this approach converges to the \emph{optimal} action-value function under Monro-Robbins conditions~\cite{NIPS1993_5807a685}.
